iNeMo: Incremental Neural Mesh Models for Robust Class-Incremental Learning

Different from human nature, it is still common practice today for vision tasks to train deep learning models only initially and on fixed datasets. A variety of approaches have recently addressed handling continual data streams. However, extending these methods to manage out-of-distribution (OOD) scenarios has not effectively been investigated. On the other hand, it has recently been shown that non-continual neural mesh models exhibit strong performance in generalizing to such OOD scenarios. To leverage this decisive property in a continual learning setting, we propose incremental neural mesh models that can be extended with new meshes over time. In addition, we present a latent space initialization strategy that enables us to allocate feature space for future unseen classes in advance and a positional regularization term that forces the features of the different classes to consistently stay in respective latent space regions. We demonstrate the effectiveness of our method through extensive experiments on the Pascal3D and ObjectNet3D datasets and show that our approach outperforms the baselines for classification by $2-6\%$ in the in-domain and by $6-50\%$ in the OOD setting. Our work also presents the first incremental learning approach for pose estimation. Our code and model can be found at https://github.com/Fischer-Tom/iNeMo.

==> data/cls_acc.tex <==
x iCarl LWF DER MEMO FOSTER Ours
0 95.0 97.25 99.0 98.0 99.2 99.8
1 92.0 91.11 95.0 91.0 97.0 99.5
2 87.0 81.03 87.0 85.0 93.0 95.8


==> data/cls_acc_Occ_1.tex <==
xocc1 Oursocc1 iCaRLocc1 LwFocc1 Podnetocc1 DERocc1 FeTrILocc1 FeCAMocc1
1 98.80	72.09	69.76	76.59 80.01 98.56 90.46
2 96.69	35.43	25.20	49.90 67.01 89.80 47.64
3 92.39	16.47	11.53	26.56 33.02 87.32 38.57
4 88.88	15.82	15.82	16.55 18.77 77.67 33.46






==> data/cls_acc_Occ_2.tex <==
xocc2 Oursocc2 iCaRLocc2 LwFocc2 Podnetocc2 DERocc2 FeTrILocc2 FeCAMocc2
1 95.57	52.79	52.79	63.09	60.83 95.16 82.32
2 92.79	22.23	17.41	36.59	48.64 78.38 34.76
3 82.65	11.67	5.93	20.76	25.04 73.76 29.16
4 77.78	17.31	10.41	11.52	12.93 57.8 24.77

==> data/cls_acc_Occ_3.tex <==
xocc3 Oursocc3 iCaRLocc3 LwFocc3 Podnetocc3 DERocc3  FeTrILocc3 FeCAMocc3
1 90.29	36.10	36.19	43.81	35.56 84.5 69.93
2 81.01	14.20	12.25	25.08	32.22 58.2 30.59
3 60.01	7.18	3.18	13.82	16.27 49.9 20.0
4 54.90	10.22	6.97	7.01	6.98 30.9 16.58

==> data/cls_acc_o3d_CI10.tex <==
x Ours iCaRL LwF Podnet DER
1 96.62	90.21	89.91	92.34	92.56
2 91.80	79.73	70.36	83.19	83.38
3 87.39	63.02	52.71	73.60	82.14
4 86.10	56.31	47.72	68.24	80.72
5 82.04	55.50	45.83	63.22	75.66
6 79.48	51.29	41.54	60.26	72.53
7 77.79	46.01	35.87	56.62	70.88
8 76.02	45.40	37.80	53.19	69.87
9 72.55	43.30	32.65	52.17	68.41
10 72.25	43.81	33.85	49.23	67.12

==> data/cls_acc_o3d_CI10_new.tex <==
x Ours iCaRL LwF Podnet DER FeTrIL FeCAM
1 97.14	90.21	89.91	92.34	92.56 95.38 97.45
2 96.94	79.73	70.36	83.19	83.38 86.86 86.1
3 94.37	63.02	52.71	73.60	82.14 81.7 79.23
4 93.24	56.31	47.72	68.24	80.72 74.56 72.73
5 90.39	55.50	45.83	63.22	75.66 68.89 67.01
6 87.18	51.29	41.54	60.26	72.53 64.53 63.48
7 85.24	46.01	35.87	56.62	70.88 61.57 60.65
8 83.81	45.40	37.80	53.19	69.87 56.96 58.37
9 80.52	43.30	32.65	52.17	68.41 56.82 56.1
10 79.67	43.81	33.85	49.23	67.12 56.14 54.81

==> data/cls_acc_o3d_CI20.tex <==
x2 Ours2 iCaRL2 LwF2 Podnet2 DER2
1 94.12	89.89	89.52 88.66	89.22
2 88.43	76.81	71.66 80.88	83.96
3 83	67.4 	60.9  69.57	76.57
4 78.29	66.93 	60.37 62.76   72.7
5 73.56	61.73	56.44 57.93   70.3

==> data/cls_acc_o3d_CI20_new.tex <==
x2 Ours2 iCaRL2 LwF2 Podnet2 DER2
1 96.18	89.89	89.52 88.66	89.22
2 92.21	76.81	71.66 80.88	83.96
3 87.85	67.4 	60.9  69.57	76.57
4 83.52	66.93 	60.37 62.76   72.7
5 80.17	61.73	56.44 57.93   70.3

==> data/cls_acc_p3d_CI3.tex <==
x2 Ours2 iCaRL2 LwF2 Podnet2 DER2
1 99.85	99.06	99.06	99.30	99.53
2 98.60	91.94	87.11	95.38	94.24
3 97.70	93.42	87.44	91.46	93.13
4 95.50	90.77	83.75	80.71	89.81

==> data/cls_acc_p3d_CI3_new.tex <==
x2 Ours2 iCaRL2 LwF2 Podnet2 DER2 FeTrIL2 FeCAM2
1 99.79	99.06	99.06	99.30	99.53 99.85 99.27
2 99.26	91.94	87.11	95.38	94.24 99.04 60.67
3 97.40	93.42	87.44	91.46	93.13 95.62 52.09
4 96.41	90.77	83.75	80.71	89.81 92.75 46.36

==> data/l1_params.tex <==
x y cls pe
0.0 0.0 93.0 85.0
0.1 1.0 95.0 83.5
0.2 1.5 94.9 83.2
0.5 2.0 95.35 82.9
1.0 2.5 95.39 82.5
1.5 3.0 95.40 81.0
2.0 3.5 95.43 80.9
2.5 4.0 95.47 80.75
3.0 4.5 95.5 80.65
3.5 5.0 95.6 79.0

==> data/l2_params.tex <==
x l1 l2
0.0 80.0 95.65
1.0 95.5 95.58
1.5 95.45 95.59
2.0 95.42 95.60
2.5 95.41 95.61
3.0 95.40 95.62
3.5 95.38 95.63
4.0 95.37 95.63
4.5 95.35 95.63
5.0 95.31 95.65

==> data/nvertices.tex <==
x acc
1130 96.0
640 95.5
250 95.3
100 95.0
50 94.0

==> data/pe_acc_p3d_CI3.tex <==
x Ours iCaRL LwF
1 74.8	37.9	38.34
2 84.2	68.8	67.84
3 80.7	60.5	49.64
4 77.4	62.2	58.06

==> data/pe_acc_p3d_pi18.tex <==
x2 Ours2 iCaRL2 LwF2
1 38.3	9.2	11.5
2 64	32.4	31.37
3 55.2	24.3	16.57
4 49.4	23.2	21.88

==> data/upperbound.tex <==
x acc
12 96.0
20 95.9
50 95.7
100 95.5
200 95.3

==> tables/classification_O3D_P3D.tex <==
{
\setlength{\tabcolsep}{1.8mm}{
\begin{table*}[tp]
  \small
  \centering
  \begin{tabu}{llccccccccc}
  \toprule
  \multirow{2.5}{*}{Metric} & & \multirow{2.5}{*}{Method} & \multirow{2.5}{*}{Repr.}&& & \multicolumn{2}{c}{\emph{P3D}} & & \multicolumn{2}{c}{\emph{O3D}}\\
  \cmidrule{7-8} \cmidrule{10-11}
  \rowfont{\scriptsize}& &    &  && & $N_{\text{task}}=2$ & $4$  &   & $5$& $10$ \\
  \midrule
    & & LWF & R50. & & & 93.83 & 89.34 & & 67.78 &48.82 \\
    Classification%\emph{Average acc.} (\%) $\uparrow$ 
    & & iCaRL & R50 & && 97.1 &  93.80 && 72.55 & 57.46\\
    \multirow{1}{*}{$acc(1\,{\colon}i)$ in \% $\uparrow$
    %$\frac{1}{N_{\text{task}}}\sum_{i=1}^{N_{\text{task}}}\mathcal{D}_{Acc}^{1:i}$
    }& & DER& R50 &&& 96.69 &  94.18 && 78.55 & 76.33\\
    & & Podnet& R50 &&& 95.13  & 91.71 & & 71.96 & 65.21\\
    & & Ours & NeMo &&& \bf{98.4} & \bf{97.91} & & \bf{83.84} & \bf{82.48}\\

  \bottomrule

    \end{tabu}
  \caption{
  Average classification accuracies on Pascal3D (P3D) and ObjectNet3D (O3D). Training data has been split into $N_{\text{task}}$ evenly distributed tasks. As visible, our method consistently outperforms the baselines by a significant margin.
  }
  \label{table: classP3DO3D}
\end{table*}
}
}
